Development of a coarse-grained water forcefield via multistate iterative Boltzmann inversion

A coarse-grained water model is developed using multistate iterative Boltzmann inversion. Following previous work, the k-means algorithm is used to dynamically map multiple water molecules to a single coarse-grained bead, allowing the use of structure-based coarse-graining methods. The model is derived to match the bulk and interfacial properties of liquid water and improves upon previous work that used single state iterative Boltzmann inversion. The model accurately reproduces the density and structural correlations of water at 305 K and 1.0 atm, stability of a liquid droplet at 305 K, and shows little tendency to crystallize at physiological conditions. This work also illustrates several advantages of using multistate iterative Boltzmann inversion for deriving generally applicable coarse-grained forcefields.

==> secs/abstract.tex <==
\begin{abstract}{}
A coarse-grained water model is developed using multistate iterative Boltzmann
inversion.
Following previous work, the $k$-means algorithm is used to dynamically map
multiple water molecules to a single coarse-grained bead, allowing the use of
structure-based coarse-graining methods.
The model is derived to match the bulk and interfacial properties of liquid
water and improves upon previous work that used single state iterative Boltzmann
inversion.
The model accurately reproduces the density and structural correlations of water
at 305~K and 1.0~atm, stability of a liquid droplet at 305 K, and shows little
tendency to crystallize at physiological conditions.
This work also illustrates several advantages of using multistate iterative
Boltzmann inversion for deriving generally applicable coarse-grained
forcefields. 
\end{abstract}

